Database of Indian Social Media Influencers on Twitter

Databases of highly networked individuals have been indispensable in studying narratives and influence on social media. To support studies on Twitter in India, we present a systematically categorised database of accounts of influence on Twitter in India, identified and annotated through an iterative process of friends, networks, and self-described profile information, verified manually. We built an initial set of accounts based on the friend network of a seed set of accounts based on real-world renown in various fields, and then snowballed "friends of friends" multiple times, and rank ordered individuals based on the number of in-group connections, and overall followers. We then manually classified identified accounts under the categories of entertainment, sports, business, government, institutions, journalism, civil society accounts that have independent standing outside of social media, as well as a category of "digital first" referring to accounts that derive their primary influence from online activity. Overall, we annotated 11580 unique accounts across all categories. The database is useful studying various questions related to the role of influencers in polarisation, misinformation, extreme speech, political discourse etc.

==> bib.tex <==
@inproceedings{inproceedings,
author = {Panda, Anmol and Gonawela, A’ndre and Acharyya, Sreangsu and Mishra, Dibyendu and Mohapatra, Mugdha and Chandrasekaran, Ramgopal and Pal, Joyojeet},
year = {2020},
month = {07},
pages = {200-209},
title = {NivaDuck - A Scalable Pipeline to Build a Database of Political Twitter Handles for India and the United States},
doi = {10.1145/3400806.3400830}
}

@inproceedings{inproceedings,
author = {Panda, Anmol and Gonawela, A’ndre and Acharyya, Sreangsu and Mishra, Dibyendu and Mohapatra, Mugdha and Chandrasekaran, Ramgopal and Pal, Joyojeet},
year = {2020},
month = {07},
pages = {200-209},
title = {NivaDuck - A Scalable Pipeline to Build a Database of Political Twitter Handles for India and the United States},
doi = {10.1145/3400806.3400830}
}

@article{Mahmud2021, 
title={Where Is This Tweet From? Inferring Home Locations of Twitter Users}, volume={6}, url={https://ojs.aaai.org/index.php/ICWSM/article/view/14299}, number={1}, journal={Proceedings of the International AAAI Conference on Web and Social Media}, author={Mahmud, Jalal and Nichols, Jeffrey and Drews, Clemens}, year={2021}, month={Aug.}, pages={511-514} }

@inproceedings{Cheng2010,
author = {Cheng, Zhiyuan and Caverlee, James and Lee, Kyumin},
title = {You Are Where You Tweet: A Content-Based Approach to Geo-Locating Twitter Users},
year = {2010},
isbn = {9781450300995},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/1871437.1871535},
doi = {10.1145/1871437.1871535},
booktitle = {Proceedings of the 19th ACM International Conference on Information and Knowledge Management},
pages = {759–768},
numpages = {10},
keywords = {text mining, twitter, location-based estimation, spatial data mining},
location = {Toronto, ON, Canada},
series = {CIKM '10}
}

@article{Al_2021, title={Homophily and Latent Attribute Inference: Inferring Latent Attributes of Twitter Users from Neighbors}, volume={6}, url={https://ojs.aaai.org/index.php/ICWSM/article/view/14340}, abstractNote={ &lt;p&gt; In this paper, we extend existing work on latent attribute inference by leveraging the principle of homophily: we evaluate the inference accuracy gained by augmenting the user features with features derived from the Twitter profiles and postings of her friends. We consider three attributes which have varying degrees of assortativity: gender, age, and political affiliation. Our approach yields a significant and robust increase in accuracy for both age and political affiliation, indicating that our approach boosts performance for attributes with moderate to high assortativity. Furthermore, different neighborhood subsets yielded optimal performance for different attributes, suggesting that different subsamples of the user’s neighborhood characterize different aspects of the user herself. Finally, inferences using only the features of a user’s neighbors outperformed those based on the user’s features alone. This suggests that the neighborhood context alone carries substantial information about the user. &lt;/p&gt; }, number={1}, journal={Proceedings of the International AAAI Conference on Web and Social Media}, author={Al Zamal, Faiyaz and Liu, Wendy and Ruths, Derek}, year={2021}, month={Aug.}, pages={387-390} }

@INPROCEEDINGS{Conover_2011,  author={Conover, Michael D. and Goncalves, Bruno and Ratkiewicz, Jacob and Flammini, Alessandro and Menczer, Filippo},  booktitle={2011 IEEE Third International Conference on Privacy, Security, Risk and Trust and 2011 IEEE Third International Conference on Social Computing},   title={Predicting the Political Alignment of Twitter Users},   year={2011},  volume={},  number={},  pages={192-199},  doi={10.1109/PASSAT/SocialCom.2011.34}}

@article{Pennacchiotti_2021, title={A Machine Learning Approach to Twitter User Classification}, volume={5}, url={https://ojs.aaai.org/index.php/ICWSM/article/view/14139}, abstractNote={ &lt;p&gt; This paper addresses the task of user classification in social media, with an application to Twitter. We automatically infer the values of user attributes such as political orientation or ethnicity by leveraging observable information such as the user behavior, network structure and the linguistic content of the user&amp;rsquo;s Twitter feed. We employ a machine learning approach which relies on a comprehensive set of features derived from such user information. We report encouraging experimental results on 3 tasks with different characteristics: political affiliation detection, ethnicity identification and detecting affinity for a particular business. Finally, our analysis shows that rich linguistic features prove consistently valuable across the 3 tasks and show great promise for additional user classification needs. &lt;/p&gt; }, number={1}, journal={Proceedings of the International AAAI Conference on Web and Social Media}, author={Pennacchiotti, Marco and Popescu, Ana-Maria}, year={2021}, month={Aug.}, pages={281-288} }

@article{Cohen_2021, title={Classifying Political Orientation on Twitter: It’s Not Easy!}, volume={7}, url={https://ojs.aaai.org/index.php/ICWSM/article/view/14434}, abstractNote={ &lt;p&gt; Numerous papers have reported great success at inferring the political orientation of Twitter users. This paper has some unfortunate news to deliver: while past work has been sound and often methodologically novel, we have discovered that reported accuracies have been systemically overoptimistic due to the way in which validation datasets have been collected, reporting accuracy levels nearly 30\% higher than can be expected in populations of general Twitter users. Using careful and novel data collection and annotation techniques, we collected three different sets of Twitter users, each characterizing a different degree of political engagement on Twitter - from politicians (highly politically vocal) to &quot;normal&quot; users (those who rarely discuss politics). Applying standard techniques for inferring political orientation, we show that methods which previously reported greater than 90\% inference accuracy, actually achieve barely 65\% accuracy on normal users. We also show that classifiers cannot be used to classify users outside the narrow range of political orientation on which they were trained. While a sobering finding, our results quantify and call attention to overlooked problems in the latent attribute inference literature that, no doubt, extend beyond political orientation inference: the way in which datasets are assembled and the transferability of classifiers. &lt;/p&gt; }, number={1}, journal={Proceedings of the International AAAI Conference on Web and Social Media}, author={Cohen, Raviv and Ruths, Derek}, year={2021}, month={Aug.}, pages={91-99} }

@inproceedings{FAIR,
author = {Wilkinson, Mark D and Dumontier, Michel and Aalbersberg, IJsbrand Jan and Appleton, Gabrielle and Axton, Myles and Baak, Arie and Blomberg, Niklas and Boiten, Jan-Willem and da Silva Santos, Luiz Bonino and Bourne, Philip E. and Bouwman, Jildau and Brookes, Anthony J. and Clark, Tim and Crosas, Mercè and Dillo, Ingrid and Dumon, Olivier and Edmunds, Scott and Evelo, Chris T. and Finkers, Richard and Gonzalez-Beltran, Alejandra and Gray, Alasdair J G and Groth, Paul and Goble, Carole and Grethe, Jeffrey S and Heringa, Jaap and ’t Hoen, Peter A C and Hooft, Rob and Kuhn, Tobias and Kok, Ruben and Kok, Joost and Lusher, Scott J and Martone, Maryann E. and Mons, Albert and Packer, Abel L and Persson, Bengt and Rocca-Serra, Philippe and Roos, Marco and van Schaik, Rene and Sansone, Susanna-Assunta and Schultes, Erik and Sengstag, Thierry and Slater, Ted and Strawn, George and Swertz, Morris A and Thompson, Mark and van der Lei, Johan and van Mulligen, Erik and Velterop, Jan and Waagmeester, Andra and Wittenburg, Peter and Wolstencroft, Katherine and Zhao, Jun and Mons, Barend},
title = {The FAIR Guiding Principles for scientific data management and stewardship},
year = {2016},
publisher = {Nature},
address = {New York, NY, USA},
url = {https://doi.org/10.1038/sdata.2016.18},
doi = {10.1038/sdata.2016.18},
booktitle = {Scientific Data},

}

@misc{dash2021divided,
      title={Divided We Rule: Influencer Polarization on Twitter During Political Crises in India}, 
      author={Saloni Dash and Dibyendu Mishra and Gazal Shekhawat and Joyojeet Pal},
      year={2021},
      eprint={2105.08361},
      archivePrefix={arXiv},
      primaryClass={cs.SI}
}

@misc{dash2021insights,
      title={Insights Into Incitement: A Computational Perspective on Dangerous Speech on Twitter in India}, 
      author={Saloni Dash and Rynaa Grover and Gazal Shekhawat and Sukhnidh Kaur and Dibyendu Mishra and Joyojeet Pal},
      year={2021},
      eprint={2111.03906},
      archivePrefix={arXiv},
      primaryClass={cs.SI}
}

@article{mothilal2022voting,
  title={Voting with the stars: Analyzing Partisan Engagement between Celebrities and Politicians in India},
  author={Kommiya Mothilal, Ramaravind and Mishra, Dibyendu and Nishal, Sachita and Lalani, Faisal and Pal, Joyojeet},
  journal={Proceedings of the ACM on Human-Computer Interaction},
  notes={to appear},
  year={2022},
  publisher={ACM New York, NY, USA}
}

%https://arxiv.org/ftp/arxiv/papers/2109/2109.07409.pdf
@misc{mishra2021sports, 
    title={Sporting the government: Twitter as a window into sportspersons’ engagement with causes in India and USA},
    author={Mishra, Dibyendu and Sen, Ronojoy and Pal, Joyojeet},
    year={2021},
    eprint={2109.07409}
}

@article{dash2021extremism,
  title={Extremism \& Whataboutism: A Case Study on Bangalore Riots},
  author={Dash, Saloni and Shekhawat, Gazal and Akbar, Syeda Zainab and Pal, Joyojeet},
  journal={arXiv preprint arXiv:2109.10526},
  year={2021}
}

@misc{DVN/F3EWLZ_2022,
author = {Arya, Arshia and De, Soham and Mishra, Dibyendu and Shekhawat, Gazal and Sharma, Ankur and Panda, Anmol and M Lalani, Faisal and Singh, Parantak and Kommiya Mothilal, Ramaravind and Grover, Rynaa and Nishal, Sachita and Dash, Saloni and Rashid Shora, Shehla and Akbar, Syeda Zainab and Pal, Joyojeet},
publisher = {Harvard Dataverse},
title = {{DISMISS: Database of Indian Social Media Influencers (Snowballed Sequentially) on Twitter}},
year = {2022},
version = {V1},
doi = {10.7910/DVN/F3EWLZ},
url = {https://doi.org/10.7910/DVN/F3EWLZ}
}

@inbook{10.1145/3460112.3471983,
author = {Arya, Arshia and Shora, Shehla Rashid and Pal, Joyojeet},
title = {Beyond Business: A Poster Contrasting CEO Activism on Social Media in India and the United States},
year = {2021},
isbn = {9781450384537},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3460112.3471983},
abstract = { We studied the Twitter activity of business leaders of top 250 companies in India and the US between January, 2019 and May, 2021 and looked for trends related to cause-related messaging through a topical analysis of their tweets. Using a Word2Vec bag of words model for textual classification, we quantified their engagement with socio-political messaging, using keywords related to the United Nations Sustainable Development Goals (UN SDGs). We found that messaging on themes that have widespread social purchase and are not politically sensitive is relatively comparable across the two countries, but that results differ vastly on issues of political sensitivity. Our results point at the complex relationship between business and politics in the two countries, and the growing importance of social media in signalling those. We conclude by pointing out the importance of these findings for political science and policy research and by highlighting the scope for future work in this area. },
booktitle = {ACM SIGCAS Conference on Computing and Sustainable Societies},
pages = {432–436},
numpages = {5}
}

